Sequential Chance Optimization For Flow-Tube Based Control Of Probabilistic Nonlinear Systems

In this paper, we address the problem of closed-loop control of nonlinear dynamical systems subjected to probabilistic uncertainties. More precisely, we design time-varying polynomial feedback controllers to follow the given nominal trajectory and also, for safety purposes, remain in the tube around the nominal trajectory, despite all uncertainties. We formulate this problem as a chance optimization problem where we maximize the probability of achieving control objectives. To address control problems with long planning horizons, we formulate the single large chance optimization problem as a sequence of smaller chance optimization problems. To solve the obtained chance optimization problems, we leverage the theory of measures and moments and obtain convex relaxations in the form of semidefinite programs. We provide numerical examples on stabilizing controller design and motion planning of uncertain nonlinear systems to illustrate the performance of the proposed approach.

==> aaai.bst.tex <==
%Filename: AAAI.bst
% BibTeX `aaai' style file for BibTeX version 0.99c, LaTeX version 2.09
% Version of 22 February 2017
% Place it in a file called aaai.bst in the BibTeX search path. (Placing it
% in the same directory as the LaTeX document should also work.)
% Support for named citations is provided by named.sty
% This version was made by modifying the master file made by
% Oren Patashnik (PATASHNIK@SCORE.STANFORD.EDU)
% Copyright (C) 1985, all rights reserved.
% Modifications Copyright (C) 1988, 1989, 1994, Peter F. Patel-Schneider
% Copying of this file is authorized only if either
% (1) you make absolutely no changes to your copy, including name, or
% (2) if you do make changes, you name it something other than
% btxbst.doc, plain.bst, unsrt.bst, alpha.bst, and abbrv.bst.
% This restriction helps ensure that all standard styles are identical.
% This style is NOT guaranteed to work. It is provided in the hope
% that it will make the preparation of papers easier.
%
% There are undoubtably bugs in this style. If you make bug fixes,
% improvements, etc. please us know (www.aaai.org)
% The preparation of this modified file was supported by Schlumberger Palo
% Alto Research and AT\&T Bell Laboratories.
% Modifications Copyright (C) 1990. Sunil Issar si@cs.cmu.edu
% Modified the file so that the Bibliography style is closer to the
% one specified in the Instructions to Authors for AAAI papers.
% This style is NOT guaranteed to work. It is provided in the hope
% that it will make the preparation of papers easier.
% Standard disclaimers apply. Send comments etc., to si@cs.cmu.edu
% This file can be used in other conferences as long as credit to the
% authors and supporting agencies is retained, this notice is not changed,
% and further modification or reuse is not restricted. 
%  Name format in citations: 
% single authorFirst
% two authorsFirst and Second
% three authorsFirst, Second, and Third
% more authorsFirst et al.
%
% Bibliography format
% author. date. other.
% Author format
% single authorFirst, Initials
% two authorsFirst, Initials, and Second, Initials
% more authorsFirst, Initials; ...; and Last, Initials
%
% Reference list ordering: alphabetical by author or whatever passes
% for author in the absence of one.
%
% This BibTeX style has support for short (year only) citations. This
% is done by having the citations actually look like
%  \citeauthoryear{author-info}{year}
% The LaTeX style has to have support for this
ENTRY
{ address
author
booktitle
chapter
edition
editor
howpublished
institution
journal
key
month
note
number
organization
pages
publisher
school
series
title
type
volume
year
}
{}
{ label extra.label sort.label }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
#1 'mid.sentence :=
#2 'after.sentence :=
#3 'after.block :=
}
STRINGS { s t }
FUNCTION {output.nonnull}
{ 's :=
output.state mid.sentence =
{ ", " * write$ }
{ output.state after.block =
{ add.period$ write$
newline$
"\newblock " write$
}
{ output.state before.all =
'write$
{ add.period$ " " * write$ }
if$
}
if$
mid.sentence 'output.state :=
}
if$
s
}
FUNCTION {sioutput.nonnull}
{ 's :=
output.state mid.sentence =
{ " " * write$ }
{ output.state after.block =
{ add.period$ write$
newline$
"\newblock " write$
}
{ output.state before.all =
'write$
{ add.period$ " " * write$ }
if$
}
if$
mid.sentence 'output.state :=
}
if$
s
}
FUNCTION {output}
{ duplicate$ empty$
'pop$
'output.nonnull
if$
}
FUNCTION {sioutput}
{ duplicate$ empty$
'pop$
'sioutput.nonnull
if$
}
FUNCTION {output.check}
{ 't :=
duplicate$ empty$
{ pop$ "empty " t * " in " * cite$ * warning$ }
'output.nonnull
if$
}
FUNCTION {output.bibitem}
{ newline$
"\bibitem[" write$
label write$
"]{" write$
cite$ write$
"}" write$
newline$
""
before.all 'output.state :=
}
FUNCTION {fin.entry}
{ add.period$
write$
newline$
}
FUNCTION {new.block}
{ output.state before.all =
'skip$
{ after.block 'output.state := }
if$
}
FUNCTION {new.sentence}
{ output.state after.block =
'skip$
{ output.state before.all =
'skip$
{ after.sentence 'output.state := }
if$
}
if$
}
FUNCTION {not}
{  { #0 }
{ #1 }
if$
}
FUNCTION {and}
{  'skip$
{ pop$ #0 }
if$
}
FUNCTION {or}
{  { pop$ #1 }
'skip$
if$
}
FUNCTION {new.block.checka}
{ empty$
'skip$
'new.block
if$
}
FUNCTION {new.block.checkb}
{ empty$
swap$ empty$
and
'skip$
'new.block
if$
}
FUNCTION {new.sentence.checka}
{ empty$
'skip$
'new.sentence
if$
}
FUNCTION {new.sentence.checkb}
{ empty$
swap$ empty$
and
'skip$
'new.sentence
if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
{ pop$ "" }
'skip$
if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
{ pop$ "" }
{ "{\em " swap$ * "}" * }
if$
}
INTEGERS { nameptr namesleft numnames }
FUNCTION {format.publisher}
{ publisher empty$
{ "" }
{ address empty$
{ publisher }
{ address ": " * publisher * }
if$ 
}
if$
}
FUNCTION {format.organization}
{ organization empty$
{ "" }
{ address empty$
{ organization }
{ address ": " * organization * }
if$ 
}
if$
}
FUNCTION {format.names}
{ 's :=
#1 'nameptr :=
s num.names$ 'numnames :=
numnames 'namesleft :=
{ namesleft #0 > }
{ s nameptr "{vv~}{ll}{, jj}{, f.}" format.name$ 't :=
nameptr #1 >
{ namesleft #1 >
{ "; " * t * }
{ numnames #2 >
{ ";" * }
{ "," * }
if$
t "others" =
{ " et~al." * }
{ " and " * t * }
if$
}
if$
}
't
if$
nameptr #1 + 'nameptr :=
namesleft #1 - 'namesleft :=
}
while$
add.period$
}
FUNCTION {format.authors}
{ author empty$
{ "" }
{ author format.names }
if$
}
FUNCTION {format.editors}
{ editor empty$
{ "" }
{ editor format.names
editor num.names$ #1 >
{ ", eds." * }
{ ", ed." * }
if$
}
if$
}
FUNCTION {format.title}
{ title empty$
{ "" }
{ title "t" change.case$ }
if$
}
FUNCTION {n.dashify}
{ 't :=
""
{ t empty$ not }
{ t #1 #1 substring$ "-" =
{ t #1 #2 substring$ "--" = not
{ "--" *
t #2 global.max$ substring$ 't :=
}
{  { t #1 #1 substring$ "-" = }
{ "-" *
t #2 global.max$ substring$ 't :=
}
while$
}
if$
}
{ t #1 #1 substring$ *
t #2 global.max$ substring$ 't :=
}
if$
}
while$
}
FUNCTION {format.year}
{ year empty$
{ "" }
{ year extra.label * }
if$
}
FUNCTION {format.date}
{ year empty$
{ month empty$
{ "" }
{ "there's a month but no year in " cite$ * warning$
month
}
if$
}
{ month empty$
'year
{ month " " * year * }
if$
}
if$
}
FUNCTION {format.btitle}
{ title emphasize
}
FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
{ "~" }
{ " " }
if$
swap$ * *
}
FUNCTION {either.or.check}
{ empty$
'pop$
{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
if$
}
FUNCTION {format.bvolume}
{ volume empty$
{ "" }
{ "volume" volume tie.or.space.connect
series empty$
'skip$
{ " of " * series emphasize * }
if$
"volume and number" number either.or.check
}
if$
}
FUNCTION {format.number.series}
{ volume empty$
{ number empty$
{ series field.or.null }
{ output.state mid.sentence =
{ "number" }
{ "Number" }
if$
number tie.or.space.connect
series empty$
{ "there's a number but no series in " cite$ * warning$ }
{ " in " * series * }
if$
}
if$
}
{ "" }
if$
}
FUNCTION {format.edition}
{ edition empty$
{ "" }
{ output.state mid.sentence =
{ edition "l" change.case$ " edition" * }
{ edition "t" change.case$ " edition" * }
if$
}
if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
#0 'multiresult :=
{ multiresult not
t empty$ not
and
}
{ t #1 #1 substring$
duplicate$ "-" =
swap$ duplicate$ "," =
swap$ "+" =
or or
{ #1 'multiresult := }
{ t #2 global.max$ substring$ 't := }
if$
}
while$
multiresult
}
FUNCTION {format.pages}
{ pages empty$
{ "" }
{ pages multi.page.check
{ "" pages n.dashify tie.or.space.connect }
{ "" pages tie.or.space.connect }
if$
}
if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null
number empty$
'skip$
{ "(" number * ")" * *
volume empty$
{ "there's a number but no volume in " cite$ * warning$ }
'skip$
if$
}
if$
pages empty$
'skip$
{ duplicate$ empty$
{ pop$ format.pages }
{ ":" * pages n.dashify * }
if$
}
if$
}
FUNCTION {format.chapter.pages}
{ chapter empty$
'format.pages
{ type empty$
{ "chapter" }
{ type "l" change.case$ }
if$
chapter tie.or.space.connect
pages empty$
'skip$
{ ", " * format.pages * }
if$
}
if$
}
FUNCTION {format.in.ed.booktitle}
{ booktitle empty$
{ "" }
{ editor empty$
{ "In " booktitle emphasize * }
{ "In " format.editors * ", " * booktitle emphasize * }
if$
}
if$
}
FUNCTION {empty.misc.check}
{ author empty$ title empty$ howpublished empty$
month empty$ year empty$ note empty$
and and and and and
key empty$ not and
{ "all relevant fields are empty in " cite$ * warning$ }
'skip$
if$
}
FUNCTION {format.thesis.type}
{ type empty$
'skip$
{ pop$
type "t" change.case$
}
if$
}
FUNCTION {format.tr.number}
{ type empty$
{ "Technical Report" }
'type
if$
number empty$
{ "t" change.case$ }
{ number tie.or.space.connect }
if$
}
FUNCTION {format.article.crossref}
{ key empty$
{ journal empty$
{ "need key or journal for " cite$ * " to crossref " * crossref *
warning$
""
}
{ "In {\em " journal * "\/}" * }
if$
}
{ "In " key * }
if$
" \shortcite{" * crossref * "}" *
}
FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
editor num.names$ duplicate$
#2 >
{ pop$ " et~al." * }
{ #2 <
'skip$
{ editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
{ " et~al." * }
{ " and " * editor #2 "{vv~}{ll}" format.name$ * }
if$
}
if$
}
if$
}
FUNCTION {format.book.crossref}
{ volume empty$
{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
"In "
}
{ "Volume" volume tie.or.space.connect
" of " *
}
if$
editor empty$
editor field.or.null author field.or.null =
or
{ key empty$
{ series empty$
{ "need editor, key, or series for " cite$ * " to crossref " *
crossref * warning$
"" *
}
{ "{\em " * series * "\/}" * }
if$
}
{ key * }
if$
}
{ format.crossref.editor * }
if$
" \shortcite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
editor field.or.null author field.or.null =
or
{ key empty$
{ booktitle empty$
{ "need editor, key, or booktitle for " cite$ * " to crossref " *
crossref * warning$
""
}
{ "In {\em " booktitle * "\/}" * }
if$
}
{ "In " key * }
if$
}
{ "In " format.crossref.editor * }
if$
" \shortcite{" * crossref * "}" *
}
FUNCTION {article}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.title "title" output.check
new.block
crossref missing$
{ journal emphasize "journal" output.check
format.vol.num.pages sioutput
}
{ format.article.crossref output.nonnull
format.pages sioutput
}
if$
new.block
note output
fin.entry
}
FUNCTION {book}
{ output.bibitem
author empty$
{ format.editors "author and editor" output.check }
{ format.authors output.nonnull
crossref missing$
{ "author and editor" editor either.or.check }
'skip$
if$
}
if$
new.block format.year "year" output.check
new.block
format.btitle "title" output.check
crossref missing$
{ format.bvolume output
new.block
format.number.series output
new.sentence
format.publisher "publisher" output.check
}
{ new.block
format.book.crossref output.nonnull
}
if$
format.edition output
% format.date "year" output.check
new.block
note output
fin.entry
}
FUNCTION {booklet}
{ output.bibitem
format.authors output
new.block format.year "year" output.check
new.block
format.title "title" output.check
howpublished address new.block.checkb
howpublished output
address output
% format.date output
new.block
note output
fin.entry
}
FUNCTION {inbook}
{ output.bibitem
author empty$
{ format.editors "author and editor" output.check }
{ format.authors output.nonnull
crossref missing$
{ "author and editor" editor either.or.check }
'skip$
if$
}
if$
new.block format.year "year" output.check
new.block
format.btitle "title" output.check
crossref missing$
{ format.bvolume output
new.block
format.number.series output
new.sentence
format.publisher "publisher" output.check
}
{ format.book.crossref output.nonnull
}
if$
format.edition output
% format.date "year" output.check
new.block
format.chapter.pages "chapter and pages" output.check
new.block
note output
fin.entry
}
FUNCTION {incollection}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.title "title" output.check
new.block
crossref missing$
{ format.in.ed.booktitle "booktitle" output.check
format.bvolume output
format.number.series output
new.sentence
format.publisher "publisher" output.check
format.edition output
%  format.date "year" output.check
new.block
format.chapter.pages output
}
{ format.incoll.inproc.crossref output.nonnull
new.block
format.chapter.pages output
}
if$
new.block
note output
fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.title "title" output.check
new.block
crossref missing$
{ format.in.ed.booktitle "booktitle" output.check
format.bvolume output
format.number.series output
format.pages output
new.block
organization empty$
{ format.publisher output }
{ format.organization output }
if$
}
{ format.incoll.inproc.crossref output.nonnull
format.pages output
}
if$
new.block
note output
fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
author empty$
{ organization empty$
'skip$
{ organization output.nonnull
address output
}
if$
}
{ format.authors output.nonnull }
if$
new.block format.year "year" output.check
new.block
format.btitle "title" output.check
author empty$
{ organization empty$
{ address new.block.checka
address output
}
'skip$
if$
}
{ organization address new.block.checkb
organization output
address output
}
if$
format.edition output
% format.date output
new.block
note output
fin.entry
}
FUNCTION {mastersthesis}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.title "title" output.check
new.block
"Master's thesis" format.thesis.type output.nonnull
school "school" output.check
address output
% format.date "year" output.check
new.block
note output
fin.entry
}
FUNCTION {misc}
{ output.bibitem
format.authors output
new.block format.year "year" output.check
title howpublished new.block.checkb
format.title output
howpublished new.block.checka
howpublished output
% format.date output
new.block
note output
fin.entry
empty.misc.check
}
FUNCTION {phdthesis}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.btitle "title" output.check
new.block
"Ph.D. Dissertation" format.thesis.type output.nonnull
school "school" output.check
address output
% format.date "year" output.check
new.block
note output
fin.entry
}
FUNCTION {proceedings}
{ output.bibitem
editor empty$
{ organization output }
{ format.editors output.nonnull }
if$
new.block format.year "year" output.check
new.block
format.btitle "title" output.check
format.bvolume output
format.number.series output
editor empty$
{ publisher empty$
{ address output }
{ format.publisher output }
if$
}
{ organization empty$
{ publisher new.sentence.checka
format.publisher output
}
{ organization new.sentence.checkb
format.organization output
}
if$
}
if$
new.block
note output
fin.entry
}
FUNCTION {techreport}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.title "title" output.check
new.block
format.tr.number output.nonnull
institution "institution" output.check
address output
% format.date "year" output.check
new.block
note output
fin.entry
}
FUNCTION {unpublished}
{ output.bibitem
format.authors "author" output.check
new.block format.year "year" output.check
new.block
format.title "title" output.check
new.block
note "note" output.check
% format.date output
fin.entry
}
FUNCTION {default.type} { misc }
MACRO {jan} {"January"}
MACRO {feb} {"February"}
MACRO {mar} {"March"}
MACRO {apr} {"April"}
MACRO {may} {"May"}
MACRO {jun} {"June"}
MACRO {jul} {"July"}
MACRO {aug} {"August"}
MACRO {sep} {"September"}
MACRO {oct} {"October"}
MACRO {nov} {"November"}
MACRO {dec} {"December"}
MACRO {acmcs} {"ACM Computing Surveys"}
MACRO {acta} {"Acta Informatica"}
MACRO {cacm} {"Communications of the ACM"}
MACRO {ibmjrd} {"IBM Journal of Research and Development"}
MACRO {ibmsj} {"IBM Systems Journal"}
MACRO {ieeese} {"IEEE Transactions on Software Engineering"}
MACRO {ieeetc} {"IEEE Transactions on Computers"}
MACRO {ieeetcad}
{"IEEE Transactions on Computer-Aided Design of Integrated Circuits"}
MACRO {ipl} {"Information Processing Letters"}
MACRO {jacm} {"Journal of the ACM"}
MACRO {jcss} {"Journal of Computer and System Sciences"}
MACRO {scp} {"Science of Computer Programming"}
MACRO {sicomp} {"SIAM Journal on Computing"}
MACRO {tocs} {"ACM Transactions on Computer Systems"}
MACRO {tods} {"ACM Transactions on Database Systems"}
MACRO {tog} {"ACM Transactions on Graphics"}
MACRO {toms} {"ACM Transactions on Mathematical Software"}
MACRO {toois} {"ACM Transactions on Office Information Systems"}
MACRO {toplas} {"ACM Transactions on Programming Languages and Systems"}
MACRO {tcs} {"Theoretical Computer Science"}
READ
FUNCTION {sortify}
{ purify$
"l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
'len :=
s #1 len substring$ =
{ s len #1 + global.max$ substring$ }
's
if$
}
FUNCTION {format.lab.names}
{ 's :=
s num.names$ 'numnames :=
numnames #1 =
{ s #1 "{vv }{ll}" format.name$ }
{ numnames #2 =
{ s #1 "{vv }{ll} and " format.name$ s #2 "{vv }{ll}" format.name$ *
}
{ numnames #3 = 
{ s #1 "{vv }{ll}, " format.name$ 
s #2 "{vv }{ll}, and " format.name$ *
s #3 "{vv }{ll}" format.name$ *
}
{ s #1 "{vv }{ll }\bgroup et al\mbox{.}\egroup " format.name$
}
if$
}
if$
}
if$
}
FUNCTION {author.key.label}
{ author empty$
{ key empty$
{ cite$ #1 #3 substring$ }
{ key }
if$
}
{ author format.lab.names }
if$
}
FUNCTION {author.editor.key.label}
{ author empty$
{ editor empty$
{ key empty$
{ cite$ #1 #3 substring$ }
{ key }
if$
}
{ editor format.lab.names }
if$
}
{ author format.lab.names }
if$
}
FUNCTION {author.key.organization.label}
{ author empty$
{ key empty$
{ organization empty$
{ cite$ #1 #3 substring$ }
{ "The " #4 organization chop.word #3 text.prefix$ }
if$
}
{ key }
if$
}
{ author format.lab.names }
if$
}
FUNCTION {editor.key.organization.label}
{ editor empty$
{ key empty$
{ organization empty$
{ cite$ #1 #3 substring$ }
{ "The " #4 organization chop.word #3 text.prefix$ }
if$
}
{ key }
if$
}
{ editor format.lab.names }
if$
}
FUNCTION {calc.label}
{ type$ "book" =
type$ "inbook" =
or
'author.editor.key.label
{ type$ "proceedings" =
'editor.key.organization.label
{ type$ "manual" =
'author.key.organization.label
'author.key.label
if$
}
if$
}
if$
duplicate$
"\protect\citeauthoryear{" swap$ * "}{" *
year field.or.null purify$ * % CHANGED - pfps - 15 Feb 1989
'label :=
year field.or.null purify$ *
sortify 'sort.label :=
}
FUNCTION {sort.format.names}
{ 's :=
#1 'nameptr :=
""
s num.names$ 'numnames :=
numnames 'namesleft :=
{ namesleft #0 > }
{ nameptr #1 >
{ "  " * }
'skip$
if$
s nameptr "{vv{ } }{ll{ }}{ ff{ }}{ jj{ }}" format.name$ 't :=
nameptr numnames = t "others" = and
{ "et al" * }
{ t sortify * }
if$
nameptr #1 + 'nameptr :=
namesleft #1 - 'namesleft :=
}
while$
}
FUNCTION {sort.format.title}
{ 't :=
"A " #2
"An " #3
"The " #4 t chop.word
chop.word
chop.word
sortify
#1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
{ key empty$
{ "to sort, need author or key in " cite$ * warning$
""
}
{ key sortify }
if$
}
{ author sort.format.names }
if$
}
FUNCTION {author.editor.sort}
{ author empty$
{ editor empty$
{ key empty$
{ "to sort, need author, editor, or key in " cite$ * warning$
""
}
{ key sortify }
if$
}
{ editor sort.format.names }
if$
}
{ author sort.format.names }
if$
}
FUNCTION {author.organization.sort}
{ author empty$
{ organization empty$
{ key empty$
{ "to sort, need author, organization, or key in " cite$ * warning$
""
}
{ key sortify }
if$
}
{ "The " #4 organization chop.word sortify }
if$
}
{ author sort.format.names }
if$
}
FUNCTION {editor.organization.sort}
{ editor empty$
{ organization empty$
{ key empty$
{ "to sort, need editor, organization, or key in " cite$ * warning$
""
}
{ key sortify }
if$
}
{ "The " #4 organization chop.word sortify }
if$
}
{ editor sort.format.names }
if$
}
FUNCTION {presort}
{ calc.label
sort.label
" "
*
type$ "book" =
type$ "inbook" =
or
'author.editor.sort
{ type$ "proceedings" =
'editor.organization.sort
{ type$ "manual" =
'author.organization.sort
'author.sort
if$
}
if$
}
if$
*
" "
*
year field.or.null sortify
*
" "
*
title field.or.null
sort.format.title
*
#1 entry.max$ substring$
'sort.key$ :=
}
ITERATE {presort}
SORT
STRINGS { longest.label last.sort.label next.extra }
INTEGERS { longest.label.width last.extra.num }
FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
#0 int.to.chr$ 'last.sort.label :=
"" 'next.extra :=
#0 'longest.label.width :=
#0 'last.extra.num :=
}
FUNCTION {forward.pass}
{ last.sort.label sort.label =
{ last.extra.num #1 + 'last.extra.num :=
last.extra.num int.to.chr$ 'extra.label :=
}
{ "a" chr.to.int$ 'last.extra.num :=
"" 'extra.label :=
sort.label 'last.sort.label :=
}
if$
}
FUNCTION {reverse.pass}
{ next.extra "b" =
{ "a" 'extra.label := }
'skip$
if$
label extra.label * "}" * 'label :=  % CHANGED - pfps 15 Feb 1989
label width$ longest.label.width >
{ label 'longest.label :=
label width$ 'longest.label.width :=
}
'skip$
if$
extra.label 'next.extra :=
}
EXECUTE {initialize.longest.label}
ITERATE {forward.pass}
REVERSE {reverse.pass}
FUNCTION {begin.bib}
{ preamble$ empty$
'skip$
{ preamble$ write$ newline$ }
if$
"\begin{thebibliography}{}" write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
"\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}

